The Minimum Wiener Connector

The Wiener index of a graph is the sum of all pairwise shortest-path distances between its vertices. In this paper we study the novel problem of finding a minimum Wiener connector: given a connected graph $G=(V,E)$ and a set $Q\subseteq V$ of query vertices, find a subgraph of $G$ that connects all query vertices and has minimum Wiener index. We show that The Minimum Wiener Connector admits a polynomial-time (albeit impractical) exact algorithm for the special case where the number of query vertices is bounded. We show that in general the problem is NP-hard, and has no PTAS unless $\mathbf{P} = \mathbf{NP}$. Our main contribution is a constant-factor approximation algorithm running in time $\widetilde{O}(|Q||E|)$. A thorough experimentation on a large variety of real-world graphs confirms that our method returns smaller and denser solutions than other methods, and does so by adding to the query set $Q$ a small number of important vertices (i.e., vertices with high centrality).

==> sections/applications.tex <==
%!TEX root=../main.tex

% BENEFITS: PARAMETER LESS, SIZE IS KEPT SMALL BY THE OBJECTIVE FUNCTION

Our algorithm produces solutions that are subgraphs connecting all query nodes but at the same time are compact with respect to extra information added (nodes and edges).
Intuitively, the size and quality of these solutions highly depend on various parameters:
\begin{itemize}
\item The number of query nodes selected
\item The location of query nodes in the graph (nodes in the same community, nodes between two or more communities, random)
\item The properties of the network (density, clustering coefficient, average path length, diameter, assortativity, etc.)
\end{itemize}
As explained next, various applications can make use of the resulting solutions.

\spara{Visualizing subgraphs in online tools:}
Often there is a need to visualize via a UI a subgraph that includes a set of selected nodes.
The visualization of such subgraphs can be for different purposes: common friends between users in a social network, common entities between possibly semantically different queries, common locations between destination points of a user(s).
Therefore, the problem is how to keep the visualization clean and easy to study from the point of view of a user, by visualizing the least possible amount of extra graph information and keeping the subgraph connected.

\spara{Finding community leaders:}
Given a community of nodes, one typical problem in network analysis is identifying the leaders of such a group.
Assuming that the query nodes of our algorithm are located within the same semantic community, the solution returned would be just a few extra nodes needed to connect the query nodes.
These added nodes are more central than the query nodes and could be playing leadership roles in the community.
This also depends on the properties of the network.
If the network is highly disassortative, then the nodes found are most likely central nodes of higher authority and status.
In a setup where the graph is a social network, such central individuals could be targeted for ad campaigns as they could expose their community to those campaigns.

\spara{Finding bridges between communities:}
Given semantically different communities in a graph, another typical problem is how to connect these communities with graph paths that would propagate information between them.
Thus, if the query nodes of our algorithm are located in different communities in the graph, the extra nodes added in the solution will be the necessary nodes to connect the query nodes across these communities.
These added nodes are bridging the (two or more) communities involved and control information flow between them.
In a setup where the graph is a social network, such bridging users could be targeted for information dissemination across different communities, or for the disruption of malware spread.
